Geometric secluded paths and planar satisfiability

We consider paths with low \emph{exposure} to a 2D polygonal domain, i.e., paths which are seen as little as possible; we differentiate between \emph{integral} exposure (when we care about how long the path sees every point of the domain) and \emph{0/1} exposure (just counting whether a point is seen by the path or not). For the integral exposure, we give a PTAS for finding the minimum-exposure path between two given points in the domain; for the 0/1 version, we prove that in a simple polygon the shortest path has the minimum exposure, while in domains with holes the problem becomes NP-hard. We also highlight connections of the problem to minimum satisfiability and settle hardness of variants of planar min- and max-SAT.

==> notes.tex <==
BELOW ARE OPEN, SOME GENERAL NOTES AND SECTION ON MAX EXPOSURE


Alexander Piltz planar 3SAT arxiv (swat18 and TCS). See implications for us (Leo). ,Eg monotone with v then c means at each clause on from one side, to from the other.
Add combinations of things: eg max VC* is still hard, but max sep VC* reduces to sep min -- check

small number of holes. Is it true that for any homotopy type, the secluded path is locally shortest? Look at the cuts of any point (there may be many now). One of them must be crossed. Is it true that the cuts crossed by the locally shortest path must be crossed by any path of the same homotopy type?



ATTEMPTS TO prove VC max2SAT from Lichtenstein
we embed the reduction showing hardness of (non-planar) max2SAT \cite{gareyMax2SAT} into Lichtenstein's \cite{planar} planarization gadget (our proof actually shows hardness of both VC-cycle and V-cycle max2SAT, giving a second proof for the latter). Specifically, the proof of hardness of (non-planar) max2SAT by reduction from (non-planar) 3SAT in \cite{gareyMax2SAT} replaces every clause $x\lor y\lor z$ with 10 clauses $x,y,z,\lnot x\lor\lnot y,\lnot y\lor\lnot z,\lnot x\lor\lnot z,z\lor\lnot w,y\lor\lnot w,z\lor\lnot w$ where $w$ is a new variable. It is easy to see that every satisfied clause in the 3SAT corresponds to (at least) 7 satisfied clauses in the max2SAT, while any unsatisfied clause in the 3SAT gives rise to strictly less than 7 satisfied 2SAT clauses.

Lichtenstein \cite{planar} proved hardness of planar 3SAT by starting from an instance of (not necessarily planar) 3SAT, building the graph which connects the variables and the clauses, and using the crossover gadget to planarize the graph. Similarly to \cite{planar}, we start from an instance of max2SAT, put the variables on a horizontal line, clauses on a horizontal line, and draw the variables--clauses graph with axis-parallel edges; see Fig.~\ref{max2sat_grid}, reproducing \cite[Fig.~6]{planar}. Then we get rid of intersections using a modification of Lichtenstein's crossover box (Fig,~\ref{planarity_gadget}): our crossover gadget is the gadget from \cite{planar} in which every clause is replaced with the 10 2SAT clauses of \cite{gareyMax2SAT}. As a result, we have a planar max2SAT instance in which it is possibly to satisfy $7|V|+7rK$ clauses, where $|V|$ is the number of variables in the original

The rest is the same as in \cite{planar}: the ability to negate literals suffices to push the assignment through the crossover gadget, removing the crossings.

\begin{figure}\centering\includegraphics[width=0.5\textwidth]{pics/grid}\caption{The overall construction with the V- and VC-cycles from \cite[Fig.~6]{planar}}\label{max2sat_grid}\end{figure}
\begin{figure}\centering\includegraphics[width=0.9\textwidth]{planarity_gadget}\caption{}\label{planarity_gadget}\end{figure}
Fig.~\ref{} shows how to run the V- and VC-cycles through our crossover gadget, proving hardness of V-cycle and VC-cycle planar min2SAT.



For the exact runtime of PTAS, could use \cite{pap} or \cite{ams05} -- if our angles are bdd. Mention can do other things with integer coordinates. T(m,M,W, angles) . W is bad, if we have non-integers; still some may have W/w, and we have $L^2/(1/2)$. Check survey and Cheng slides; see what we can guarantee.

For the hardness of WRP, %The survey says if predicates can be done exactly, MiPa gives exact answer. The slides http://www.iitg.ac.in/rinkulu/talks/spweireg.pdf for an unpublished paper says it's believed to be hard

OLD: Triangles with both sides fixed-endpoint are easy to handle (Fig.~\ref{refine}, left), as for them the level sets degenerate to straight lines running parallel to the base at heights forming geometric progression with the common ratio 1+\eps (for a triangle $pqr$ the level set $\gamma_A$ is the line at height $2A/|qr|$ above $qr$). As above, any point sees at least the area 1/2. Thus, the first strip may have width $(1+\eps)/(2n|qr|)$ and we may assume that any point \p inside the strip sees area (1+\eps)/(4n) -- this will be at most factor 1+\eps larger than what a point on the optimal path sees; in general, the $i$th strip will have the upper boundary at ordinate $(1+\eps)^i/|qr|$ and \e{weight} $(1+\eps)^i/2$ -- such a weight will be at most factor 1+\eps larger than the area $|pqr|$ for \p on the optimal path, while the path goes through the strip. Since the strips do not need to run higher than \L from the base, the number of necessary strips is at most $\log_{1+\eps}(L|qr|)=O(\frac1\eps\log\L)$ since $|qr|\le\L$. We call the above-defined strips \e{canonical}.%(In practice, instead of the universal lower bound of 1/2 on the visible area, one may find the point \p that sees the least and use |\V\p| for the bound.)
\begin{figure}\centering\caption{Left: $|pqr|=y|pr|/2$, assuming $pr$ is on the x-axis; the weight of the stip of \p is $(1+\eps)^i/2=(1+\eps)\left(1/2\cdot(1+\eps)^{i-1}/|qr|\cdot|qr|\right)\le(1+\eps)|pqr|$. Middle: The edges of the refinement of the visibility decomposition are dotted}\label{refine}\end{figure}
canonical strips also for edges of VG
There exist domains in which $O(n^4)$ cells of the visibility decomposition have $O(n)$ complexity (Fig.~\ref{n5}); thus our overall approach cannot probably be made much faster.

[PERHAPS NO NEED]\item In \cite{luckow}, the following variant of the problem (dubbed \e{short} secluded \s-\t path) was proved to be hard: given \e{two} numbers $(l,k)$, does there exist an \s-\t path that has at most $l$ vertices and is adjacent to at most $k$ vertices (the difference from the vanilla \sc is that the vertices of the path itself are \e{not} counted as adjacent to the path). This variant can also be seen hard by our reduction from min2SAT (Fig.~\ref{graph}), since the path goes through exactly $n$ vertices.  % is proved hard in https://arxiv.org/pdf/1212.6176.pdf  and can also be seen hard by our reduction from min2SAT. also in planar

In \cite{chechik}, the original vertices may have degree 3: while in the graph version it does not matter how many times (1,2 or 3) the path is adjacent to an unforced vertex $v$, in our geometric case it could be tedious to ensure that the extra area seen does not change much depending on whether the area, corresponding to $v$, is seen from 1, 2 or 3 forced vertex gadgets. We therefore chose to reduce from min2SAT.



\section{Maximum exposure}\label{smax}
We now flip the objective and look for paths which see as much as possible. \e{Maximization} of path exposure in geometric domains is the subject in \e{watchman route problems} \cite{bengt,csaba,apx,eli,touring} where the goal is to find the shortest loop from which every point of the domain is seen; visiting a maximum set of points in the plane (without obstacles) with a bounded-length tour is the orienteering/prize-collecting TSP \cite{}. Speak about bdd-length max area and show the folklore reduction showing hardness even in simple polygons (and scaling since we use it later?)?
Take from below that we look for a cycle and have no starting point for the maximization version

For the maximum exposure we make two technical assumptions:
a bound \L on the path length is given in the input (without the bound, i.e., allowing arbitrary-length paths, the problem is void).
As our problem is a generalization of WRP, we look for a maximum-exposure \e{cycle} (this is the standard setting in WRP). In particular, the no point on the cycle is given in the input (for WRP, there are fine distinctions between the standard setting and the versions with a given point on the cycle, as well as with \e{path} versions)
%the starting point \s of the path is given, but the other endpoint is not specified. (For WRP, the algorithms for the "fixed-source" version run faster by approximately a linear factor \cite{touring} then for the "floating" version, in which no point on the route is specified and, essentially, every vertex of the domain is tried as a possible \s; however, the distinction does not influence polynomial-time solvability)

Maximum integral exposure, perhaps, does not make sense, as it allows for pathological solutions in which the path may stay in a point \p of high visibility (a point with large $|\V(p)|$), ``gathering for free'' the integral visibility.

max
     simple domains
Area  hard
V      ??   hard


Look at the seen subpolygon. Wlog  Opt won't bend at a new cut (if it does, there oiginsl cut). Prove that original cuts visits in order (possibly with skips). Maintain on last step SPM per … How many? Who's last or smth

In \cite{touring}, Dror et al.\ presented an approach to WRP based on propagating the shortest-paths information from \s through the essential cuts. While the full shortest-paths map (the decomposition of \P such for any point \p within a cell of the decomposition the shortest path \s-\p path through the cuts visits each cut in the same way -- going through the cut, refletting off the cut, or bending at a cut endpoint) may have exponential complexity,

Let $P'\subseteq\P$ denote the polygon actually seen by opt; P' is a simple polygon because it is connected (via any two points in P' are connected via opt and there are no holes -- prove that area seen by a path in a simple polygon has no holes).
We have to keep all cuts, not only essential, because a non-essential cut may become essential in P'.

Joe. DP for visiting in l1 max number of chords

Below are comments from e.tex:

%%transposed tables, too wide \begin{table}\centering\begin{minipage}[c]{.3\columnwidth}\begin{tabular}{|c|c|c|}\hline
%& With holes & Simple \\\hline
%0/1 & Hard (Thm.~\ref{tmin}) &P (Thm.~\ref{tsimple}) \\\hline
%Integral & \multicolumn{2}{|c|}{PTAS (Thm.~\ref{t:ptas})}\\\hline\end{tabular}\caption{Results on minimum-exposure paths in polygonal domains}\label{results:secluded}\end{minipage}\hfill
%\begin{minipage}[c]{.7\columnwidth}\begin{tabular}{|c|c|c|c|c|}\hline
%&V-cycle & VC-cycle & Separable & Monotone\\\hline
%min2SAT & Hard (Thm.~\ref{t:opt2sat})&Open &P (Thm.~\ref{t:separable:min}) & P (Thm.~\ref{c:monotone:min})\\\hline
%max2SAT&\multicolumn{4}{|c|}{Hard (Thm.~\ref{t:opt2sat})}\\\hline
%\end{tabular}\caption{Results on versions of opt2SAT (see Section~\ref{2sat} for definitions)}\label{results:opt2sat}\end{minipage}\end{table}



==> p/README <==
    The \thmtools\ bundle provides several packages for commonly-needed 
    features for theorems. As designed, the bundle should work with kernel
    theorems, the theorem package and the amsthm package.
    
    WARNING: Currently, things might still be a bit rough. You
    might want to consider not relying on \thmtools\ for your Ph.D. thesis
    masterpiece.
    
Provided features:
a keyval interface to \newtheorem
a \listoftheorem command
hyperref/autoref compatibility
a way of restating entire theorems with a single macro call

License: LPPL 1.3a; maintained by ulmi@absatzen.de
$Id: README,v 1.1 2008/02/17 21:13:58 ulmi Exp ulmi $


==> p/VERSION.tex <==
\def\x #1-#2-#3 #4 v#5\@{\def\VERSION{#1/#2/#3 v#5}}\x 2014-04-21 20:11:26 +0200 v66\@
